Beyond Harassment: Exploring the Harm Experienced by People with Disabilities in Social Virtual Reality

People with disabilities (PWD) are increasingly engaging in social virtual reality (VR) platforms, where immersive and embodied interactions can intensify negative experiences. While prior work has examined harassment in VR, little is known about the harms experienced by PWD and the perceived severity associated with different harassment and disability types. Unlike harassment, which represents behaviors, harm is more critical to designing effective protections, as it reflects the consequences and impact; the realism of VR and the vulnerability resulting from disability identity can further amplify such impact. To characterize and model harms for PWD, we conducted a literature review, followed by an online survey with 67 PWD to understand participants' harassment experiences and resulting harms in social VR. We identified 19 types of harm in 5 categories, and reported the severity perception of each type of harm. Finally, we analyzed our results from the critical disability theory perspective, summarized the uniqueness of harm in social VR, and discussed design implications for specialized safety mechanisms that mitigate harm for PWD.

==> table/harassment-fre.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\linewidth]{images/vis_harm.png}
  \caption{ Frequency of each harm subtype, grouped by high-level harm categories.}
   % \Description{Bar chart showing distributions of harassment type for each harm type.}\yaxing{this one should go into appendix}
  \label{fig:vis_harm}
\end{figure*}
